Functional Programming in Learning Electromagnetic Theory

Electromagnetic theory is central to physics. An undergraduate major in physics typically takes a semester or a year of electromagnetic theory as a junior or senior, and a graduate student in physics typically takes an additional semester or year at a more advanced level. In fall 2023, the author taught his undergraduate electricity and magnetism class using numerical methods in Haskell in parallel with traditional analytical methods. This article describes what functional programming has to offer to physics in general, and electromagnetic theory in particular. We give examples from vector calculus, the mathematical language in which electromagnetic theory is expressed, and electromagnetic theory itself.

==> eptcsdata.tex <==
\providecommand{\firstpage}{20}
\providecommand{\publicationstatus}{Stephen Chang (Ed.): Trends in Functional\\ Programming in Education (TFPIE)
\\
EPTCS 405, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.405.2}{10.4204/EPTCS.405.2}}
\pdfoutput=1

